Life time of topological coherent modes of a Bose--Einstein condensate in a gravito optical surface trap

We give numerical estimates of various unstable stationary solutions of the Gross--Pitaevskii equation in an axially symmetric set up with a linear trapping potential along the symmetry axis, and a quadratic trapping along the radial direction. These represent topological coherent modes of Bose--Einstein condensates in a gravito optical surface trap (GOST). Despite their instability, we find that many of these solutions decay sufficiently slow, so that they could be realized experimentally.

==> appa.tex <==
\section{Half-life time fit data} \label{sec:app_fit_data}

Fitting Function: $\exp \lambda t+c$.

$\tau_{1/2} \equiv \ln 2 / \lambda$

\subsection{A1}
\begin{footnotesize}
\csvreader[no head, tabular={lcccccc}, table head=\hline$N$ & $\lambda$ & $c$ & $\sigma^2_c$ & $\rho(\lambda c)$ & $\sigma^2_{\lambda}$ & $\chi^2$ \\\hline, table foot=\hline]{csv/1_0_0_fits.csv}{1=\eins,2=\zwei,3=\drei,4=\vier,5=\fuenf,6=\sechs,7=\sieben,8=\acht}{\eins & \drei & \vier & \fuenf & \sechs & \sieben & \acht}
\end{footnotesize}

\subsection{A2}
\begin{footnotesize}
\csvreader[no head, tabular={lcccccc}, table head=\hline$N$ & $\lambda$ & $c$ & $\sigma^2_c$ & $\rho(\lambda c)$ & $\sigma^2_{\lambda}$ & $\chi^2$ \\\hline, table foot=\hline]{csv/2_0_0_fits.csv}{1=\eins,2=\zwei,3=\drei,4=\vier,5=\fuenf,6=\sechs,7=\sieben,8=\acht}{\eins & \drei & \vier & \fuenf & \sechs & \sieben & \acht}
\end{footnotesize}

\subsection{A3}
\begin{footnotesize}
\csvreader[no head, tabular={lcccccc}, table head=\hline$N$ & $\lambda$ & $c$ & $\sigma^2_c$ & $\rho(\lambda c)$ & $\sigma^2_{\lambda}$ & $\chi^2$ \\\hline, table foot=\hline]{csv/0_1_0_fits.csv}{1=\eins,3=\drei,4=\vier,5=\fuenf,6=\sechs,7=\sieben,8=\acht}{\eins & \drei & \vier & \fuenf & \sechs & \sieben & \acht}
\end{footnotesize}

\subsection{B1}
\begin{footnotesize}
\csvreader[no head, tabular={lcccccc}, table head=\hline$N$ & $\lambda$ & $c$ & $\sigma^2_c$  & $\rho(\lambda c)$& $\sigma^2_{\lambda}$ & $\chi^2$ \\\hline, table foot=\hline]{csv/1_0_1_fits.csv}{1=\eins,2=\zwei,3=\drei,4=\vier,5=\fuenf,6=\sechs,7=\sieben,8=\acht}{\eins & \drei & \vier & \fuenf & \sechs & \sieben & \acht}
\end{footnotesize}

\subsection{B2}
\begin{footnotesize}
\csvreader[no head, tabular={lcccccc}, table head=\hline$N$ & $\lambda$ & $c$ & $\sigma^2_c$ & $\rho(\lambda c)$ & $\sigma^2_{\lambda}$ & $\chi^2$ \\\hline, table foot=\hline]{csv/2_0_1_fits.csv}{1=\eins,2=\zwei,3=\drei,4=\vier,5=\fuenf,6=\sechs,7=\sieben,8=\acht}{\eins & \drei & \vier & \fuenf & \sechs & \sieben & \acht}
\end{footnotesize}

\subsection{B3}
\begin{footnotesize}
\csvreader[no head, tabular={lcccccc}, table head=\hline$N$ & $\lambda$ & $c$ & $\sigma^2_c$ & $\rho(\lambda c)$ & $\sigma^2_{\lambda}$ & $\chi^2$ \\\hline, table foot=\hline]{csv/0_1_1_fits.csv}{1=\eins,2=\zwei,3=\drei,4=\vier,5=\fuenf,6=\sechs,7=\sieben,8=\acht}{\eins & \drei & \vier & \fuenf & \sechs & \sieben & \acht}
\end{footnotesize}

==> hudef.tex <==
\def\hdir{/home/hannes/su-book/npde}
\def\pdir{/home/hannes/su-book/npde/pictures}
\def\pdirb{/home/hannes/su-book/npde/pictures2}
\def\pdirc{/home/hannes/su-book/npde/pics3}
\def\exdir{/home/hannes/su-book/npde/exercises}
\def\exdirb{/home/hannes/su-book/npde/exercises2}
\def\soldir{/home/hannes/su-book/npde/solutions}
\def\soldirb{/home/hannes/su-book/npde/solutions2}
\def\sdir{/home/hannes/su-book/npde/skript1}
\def\sdirb{/home/hannes/su-book/npde/skript2}

\def\bexe{\begin{exercise}}\def\eexe{\eex\end{exercise}}
\def\bsol{\begin{solution}}\def\esol{\eex\end{solution}}
\def\bexa{\begin{example}}\def\eexa{\eex\end{example}}
\def\brem{\begin{remark}}\def\erem{\eex\end{remark}}

%%%%%%%%%%%%%%%%%%%%%% Hannes Def %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\newcommand{\R}{{\mathbb R}}
\newcommand{\C}{{\mathbb C}}\newcommand{\N}{{\mathbb N}}
\newcommand{\Q}{{\mathbb Q}}\newcommand{\Z}{{\mathbb Z}}

\def\CC{{\cal C}}\def\CK{{\cal K}}\def\CT{{\cal T}}\def\CU{{\cal U}}
\def\CV{{\cal V}}\def\CA{{\cal A}}\def\CE{{\cal E}}\def\CD{{\cal D}}  
\def\CF{{\cal F}}\def\CG{{\cal G}}\def\CH{{\cal H}}\def\CL{{\cal L}}
\def\CO{{\cal O}}\def\CP{{\cal P}}\def\CR{{\cal R}}\def\CS{{\cal S}}
\def\CM{{\cal M}}\def\CN{{\cal N}}\def\CZ{{\cal Z}}\def\CB{{\cal B}}

\def\ga{\gamma}\def\om{\omega}\def\th{\theta}\def\uh{\hat{u}}\def\vh{\hat{v}}
\def\noi{\noindent}\def\ds{\displaystyle}
\def\vt{\vartheta}\def\Id{\mbox{Id}}\def\pa{{\partial}}\def\lam{\lambda}
\newcommand{\bi}{\begin{itemize}}\newcommand{\ei}{\end{itemize}}
\newcommand{\bce}{\begin{center}}\newcommand{\ece}{\end{center}}
\newcommand{\reff}[1]{(\ref{#1})}\newcommand{\ul}[1]{{\underline {#1}}}
\newcommand{\mbf}[1]{{\mathbf{#1}}}\newcommand{\ov}[1]{{\overline {#1}}}
\newcommand{\ol}[1]{{\overline {#1}}}\newcommand{\nonu}{\nonumber}
\newcommand{\hs}[1]{{\hspace{#1}}}\newcommand{\vs}[1]{{\vspace{#1}}}
\def\eps{\varepsilon}\def\epsi{\epsilon}\def\aqui{\Leftrightarrow}
\def\ra{\rightarrow}\def\Ra{\Rightarrow}\def\la{\leftarrow}
\def\lra{\leftrightarrow}\def\lora{\longrightarrow}\def\loma{\longmapsto}
\newcommand{\barr}{\begin{array}}\newcommand{\earr}{\end{array}}
\newcommand{\bpm}{\begin{pmatrix}}\newcommand{\epm}{\end{pmatrix}}
\newcommand{\ba}{\begin{array}}\newcommand{\ea}{\end{array}}
\def\dd{\, {\rm d}}\def\ri{{\rm i}}\def\sech{{\rm sech}}
\def\dx{\, {\rm d}x}
\def\cc{{\rm c.c.}}\def\res{{\rm Res}}\def\er{{\rm e}}
\def\re{{\rm Re}}\def\im{{\rm Im}}\def\ccf{{\rm c.c.f}}
\def\spec{{\rm spec}}\def\om{\omega}\def\Om{\Omega}
\def\hot{{\rm h.o.t}}\def\ddt{\frac{\rm d}{{\rm d}t}}
\def\ddx{\frac{\rm d}{{\rm d}x}}\def\bphi{\varphi}\def\del{\delta}
\def\supp{{\rm supp}}


\def\nab{\nabla}\def\eex{\hfill\mbox{$\rfloor$}}
%\def\qed{\hfill $\Box$}
\def\Del{\Delta}\def\na{\nabla}
\def\phiti{\tilde{\phi}}\def\psiti{\tilde{\psi}}
\def\kti{\tilde{k}}\def\sig{\sigma}
\def\nag{\nabla{\gamma}}\def\lap{\Delta}\def\al{\alpha}
\def\fti{\tilde{f}}\def\gti{\tilde{g}}\def\wti{\tilde{w}}
\def\he{\hat{e}}\def\hemu{\hat{e}_{(\mu)}}\def\henu{\hat{e}_{(\nu)}}
\def\hemp{\hat{e}_{(\mu')}}\def\henp{\hat{e}_{(\nu')}}
\def\mup{{\mu'}}\def\nup{{\nu'}}

\def\Ga{\Gamma}\def\Rti{\tilde{R}}\def\Lam{\Lambda}
\def\kap{\kappa}\def\Sig{\Sigma}
\def\rot{\nabla\times}\def\nati{\nabla\times}\def\nad{\nabla\cdot}

\def\xmin{{x_{\mbox{\small min}}}}\def\xmax{{x_{\mbox{\small max}}}} 
\def\un{u^{(0)}}\def\ue{u^{(1)}} \def\us{{\tilde{u}}}
\def\bd{\begin{displaymath}} \def\ed{\end{displaymath}}
\def\ba{\begin{array}} \def\ea{\end{array}}
\def\ua{u^{(1)}} \def\ub{u^{(2)}}\def\uta{u_t^{(1)}} \def\utb{u_t^{(2)}}
\def\eps{\varepsilon} \def\dt{\Delta t \;}
\def\lp{\Delta} \def\cd{(t,\cdot)}\def\cn{(0,\cdot)} \def\di{\displaystyle}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% THEOREM 
\newtheorem{theorem}{Theorem}[section]
\newtheorem{definition}[theorem]{Definition}
\newtheorem{Definition}[theorem]{Definition}
\newtheorem{lemma}[theorem]{Lemma}
\newtheorem{Lemma}[theorem]{Lemma}
\newtheorem{exercise}[theorem]{Exercise}
\newtheorem{solution}[theorem]{Solution}
\newtheorem{remark}[theorem]{Remark}
\newtheorem{corollary}[theorem]{Corollary}
\newtheorem{example}[theorem]{Example}
\newtheorem{proposition}[theorem]{Proposition}

%%% Local Variables: 
%%% mode: latex
%%% TeX-master: t
%%% End: 

